NLP4RE Tools: Classification, Overview, and Management

Tools constitute an essential contribution to natural language processing for requirements engineering (NLP4RE) research. They are executable instruments that make research usable and applicable in practice. In this chapter, we first introduce a systematic classification of NLP4RE tools to improve the understanding of their types and properties. Then, we extend an existing overview with a systematic summary of 126 NLP4RE tools published between April 2019 and June 2023 to ease reuse and evolution of existing tools. Finally, we provide instructions on how to create, maintain, and disseminate NLP4RE tools to support a more rigorous management and dissemination.

==> material/bibliography.tex <==
\begin{thebibliography}{8}

\bibitem{zhao21NLP}
Zhao, L., Alhoshan, W., Ferrari, A., Letsholo, K. J., Ajagbe, M. A., Chioasca, E. V., and Batista-Navarro, R. T. (2021). Natural language processing for requirements engineering: A systematic mapping study. ACM Computing Surveys (CSUR), 54(3), 1-41.

\bibitem{frattini23recovery}
Frattini, J., Montgomery, L., Fucci, D., Fischbach, J., Unterkalmsteiner, M., Mendez, D. (2023). Let's Stop Building at the Feet of Giants: Recovering unavailable Requirements Quality Artifacts. Submitted to 2023 REFSQ Workshops.

%\bibitem{ref_url1}
%LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4 Oct 2017
\end{thebibliography}
